Slicing the cool circumgalactic medium along the major-axis of a star-forming galaxy at $z = 0.7$

We present spatially-resolved echelle spectroscopy of an intervening MgII-FeII-MgI absorption-line system detected at $z_{\rm abs}=0.73379$ toward the giant gravitational arc PSZ1 G311.65-18.48. The absorbing gas is associated to an inclined disk-like star-forming galaxy, whose major axis is aligned with the two arc-segments reported here. We probe in absorption the galaxy's extended disk continuously, at $\approx 3$ kpc sampling, from its inner region out to $15\times$ the optical radius. We detect strong ($W_0^{2796}>0.3$ \r{A}) coherent absorption along $13$ independent positions at impact parameters $D=0$--$29$ kpc on one side of the galaxy, and no absorption at $D=28$--$57$ kpc on the opposite side (all de-lensed distances at $z_{\rm abs}$). We show that: (1) the gas distribution is anisotropic; (2) $W_0^{2796}$, $W_0^{2600}$, $W_0^{2852}$, and the ratio $W_0^{2600}\!/W_0^{2796}$, all anti-correlate with $D$; (3) the $W_0^{2796}$-$D$ relation is not cuspy and exhibits significantly less scatter than the quasar-absorber statistics; (4) the absorbing gas is co-rotating with the galaxy out to $D \lesssim 20$ kpc, resembling a `flat' rotation curve, but at $D\gtrsim 20$ kpc velocities decline below the expectations from a 3D disk-model extrapolated from the nebular [OII] emission. These signatures constitute unambiguous evidence for rotating extra-planar diffuse gas, possibly also undergoing enriched accretion at its edge. Arguably, we are witnessing some of the long-sought processes of the baryon cycle in a single distant galaxy expected to be representative of such phenomena.

==> out_table.tex <==
1&-4.0&74.4$\pm$5.7&1.48$\pm$0.19&1.75$\pm$0.2&1.28$\pm$0.47\\
2&1.0&108.9$\pm$3.8&2.19$\pm$0.15&2.05$\pm$0.12&58.81$\pm$6.78\\
3&2.7&120.7$\pm$4.1&2.17$\pm$0.31&1.53$\pm$0.16&0.48$\pm$0.15\\
4&6.0&128.0$\pm$2.8&2.04$\pm$0.27&1.48$\pm$0.2&0.44$\pm$0.13\\
5&9.3&124.3$\pm$2.1&1.63$\pm$0.18&0.91$\pm$0.08&0.42$\pm$0.09\\
6&12.6&99.1$\pm$2.9&1.15$\pm$0.12&0.72$\pm$0.05&0.16$\pm$0.06\\
7&15.9&104.1$\pm$2.4&0.91$\pm$0.13&0.53$\pm$0.05&0.17$\pm$0.05\\
8&19.2&107.9$\pm$4.5&0.52$\pm$0.1&0.28$\pm$0.04&$<$0.1\\
9&22.4&101.0$\pm$13.3&0.36$\pm$0.04&$<$0.14&$<$0.11\\
10&25.8&55.9$\pm$7.8&0.49$\pm$0.04&$<$0.24&$<$0.0\\
11&29.2&41.2$\pm$7.1&0.36$\pm$0.05&$<$0.16&$<$0.11\\

